Apprentice for Event Generator Tuning

Apprentice is a tool developed for event generator tuning. It contains a range of conceptual improvements and extensions over the tuning tool Professor. Its core functionality remains the construction of a multivariate analytic surrogate model to computationally expensive Monte-Carlo event generator predictions. The surrogate model is used for numerical optimization in chi-square minimization and likelihood evaluation. Apprentice also introduces algorithms to automate the selection of observable weights to minimize the effect of mis-modeling in the event generators. We illustrate our improvements for the task of MC-generator tuning and limit setting.

==> Makefile <==
TEXROOT=main
TEXFILES=apprenticeImpact.tex \
apprenticeProblems.tex \
apprenticeUse.tex \
conclusion.tex \
introduction.tex \
macros.tex \
main.tex

SuppTEXFILES= 
PICS=
EPSS=
BIBFILES=NLP.bib \
bibliography.bib \
hep.bib \
jshort.bib \
minlp.bib \
ndrathep.bib \
ra.bib \
robust.bib

all: $(TEXROOT).pdf

# latex & bibtex main file
$(TEXROOT).pdf: $(TEXFILES) $(PICS) $(BIBFILES)
	pdflatex $(TEXROOT).tex \
	bibtex $(TEXROOT) \
	pdflatex $(TEXROOT).tex \
	bibtex $(TEXROOT) \
	pdflatex $(TEXROOT).tex \

# create pictures, if needed
.SUFFIXES: .fig .pdf

#.fig.pdf:
#	fig2dev -L pdf $< $@

clean:
	rm -f $(TEXROOT).pdf *.aux *.bbl *.blg *.toc *.log *.bak *.out *.thm *synctex.gz *~

reallyclean: clean
	rm -f pics/*.pdf


